AAA: Triple-adaptive Bayesian designs for the identification of optimal dose combinations in dual-agent dose-finding trials

We propose a flexible design for the identification of optimal dose combinations in dual-agent dose-finding clinical trials. The design is called AAA, standing for three adaptations: adaptive model selection, adaptive dose insertion, and adaptive cohort divi- sion. The adaptations highlight the need and opportunity for innovation for dual-agent dose finding, and are supported by the numerical results presented in the proposed simulation studies. To our knowledge, this is the first design that allows for all three adaptations at the same time. We find that AAA improves the statistical inference, enhances the chance of finding the optimal dose combinations, and shortens the trial duration. A clinical trial is being planned to apply the AAA design.

==> sc11_own.tex <==
\hline \hline
\multicolumn{7}{c}{\textbf{Scenario 6} \% early stop: 0.001} \\
\multicolumn{7}{l}{\textit{1.} Description }\\
\hline \hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(-1.46,0.77,1.39)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	-1.427(0.379)	&	0.86(0.703)	&	1.164(0.71)	\\	
\hline \hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(0.3,3.1,1.55,.,.)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	0.237(0.434)	&	3.226(1.123)	&	1.696(1.033)	&	.	&	.	\\	
Quadratic of agent A	&	&	-0.02(0.683)	&	7.546(2.633)	&	1.894(1.172)	&	-8.485(3.304)	&	.	\\	
Quadratic of agent B	&	&	0.41(0.581)	&	3.936(1.426)	&	3.709(1.765)	&	.	&	-7.52(2.633)	\\	
Quadratic of both agents	&	&	-0.294(0.827)	&	10.201(3.523)	&	5.628(2.276)	&	-10.653(4.515)	&	-8.081(3.232)	\\	
\hline \hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 70.3 \%$	&	\multicolumn{2}{c}{$ 13.3 \%$}	&	\multicolumn{2}{c}{$ 12.6 \%$}	&	\multicolumn{2}{c}{$ 3.7 \%$}	\\	
\hline \hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.1	&	0.4	&	0.7	&	1	&	&	\\	
0.1	&	0.06/0.08&	0.1/0.14&	0.16/0.23&	0.25/0.35&&\\
0.4	&	0.08/0.23&	0.13/0.35&	0.21/0.5&	0.31/0.65&&\\
0.7	&	0.11/0.5&	0.17/0.65&	0.26/0.77&	0.38/0.86&&\\
1	&	0.14/0.77&	0.22/0.86&	0.32/0.92&	0.45/0.95&&\\
\hline \hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(1.384,0.05),   BMS:\%ins=32.2\% }\\
\multicolumn{7}{c}{Dose inserted: 1.174(0.511), 0.256(0.25);  Dose selected: 1.002(0.367), 0.341(0.316)}\\
\hline
Dose Level(A$\backslash$B)	&	0.1	&	0.4	&	0.7	&	1	&	Dose inserted	&	Dose selected	\\
0.1	&	0.031/0.003	&	0.002/0	&	0.009/0.002	&	0.015/0.012	&	0.079/0.202	&	0.287/	\\
0.4	&	0.003/0.002	&	0.04/0.001	&	0.06/0.02	&	0.038/0.053	&	&	\\
0.7	&	0.036/0.023	&	0.118/0.052	&	0.137/0.064	&	0.028/0.034	&	&	\\
1	&	0.184/0.32	&	0.128/0.168	&	0.033/0.021	&	0.059/0.023	&	&	\\
\hline \hline
\\ \\


==> sc1_own.tex <==
\hline
\multicolumn{7}{c}{\textbf{Scenario 1} \% early stop: 0} \\
\multicolumn{7}{l}{\textit{1.} Quadratic; Efficacy peaks in the left side of MTD; Insertion is needed.}\\
\hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(-1.58,1.4,1.06)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	-1.546(0.315)	&	1.161(0.874)	&	1.041(0.823)	\\	
\hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(1.45,0.7,0.59,-9.8,-7.29)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	NaN(NaN)	&	NaN(NaN)	&	NaN(NaN)	&	.	&	.	\\	
Quadratic of agent A	&	&	1.475(0.549)	&	0.464(1.661)	&	0.917(1.278)	&	-22.318(8.56)	&	.	\\	
Quadratic of agent B	&	&	1.195(0.439)	&	1.459(1.368)	&	-0.256(1.589)	&	.	&	-23.177(8.323)	\\	
Quadratic of both agents	&	&	1.535(0.523)	&	0.527(1.56)	&	0.437(1.544)	&	-13.758(6.928)	&	-11.861(6.021)	\\	
\hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 0 \%$	&	\multicolumn{2}{c}{$ 5.8 \%$}	&	\multicolumn{2}{c}{$ 3.7 \%$}	&	\multicolumn{2}{c}{$ 90.5 \%$}	\\	
\hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.05	&	0.35	&	0.65	&	1	&	&	\\	
0.1	&	0.05/0.01&	0.07/0.1&	0.1/0.14&	0.16/0.02&&\\
0.3	&	0.07/0.12&	0.11/0.56&	0.15/0.64&	0.21/0.17&&\\
0.6	&	0.13/0.19&	0.18/0.7&	0.24/0.76&	0.33/0.27&&\\
0.9	&	0.21/0.01&	0.28/0.1&	0.37/0.14&	0.48/0.02&&\\
\hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(0.441,0.476),   BMS:\%ins=59.3\% }\\
\multicolumn{7}{c}{Dose inserted: 0.43(0.111), 0.448(0.142);  Dose selected: 0.456(0.109), 0.464(0.118)}\\
\hline
Dose Level(A$\backslash$B)	&	0.05	&	0.35	&	0.65	&	1	&	Dose inserted	&	Dose selected	\\
0.1	&	0.031/0	&	0.011/0.003	&	0.009/0.001	&	0.001/0	&	0.257/0.559	&	0.43/	\\
0.3	&	0.01/0.001	&	0.162/0.086	&	0.115/0.098	&	0.006/0.001	&	&	\\
0.6	&	0.017/0.01	&	0.189/0.184	&	0.09/0.054	&	0.02/0.002	&	&	\\
0.9	&	0.001/0	&	0.004/0.001	&	0.019/0	&	0.058/0	&	&	\\
\hline
\multicolumn{7}{l}{\textit{7.} Dose Allocation and Selection Percentages for Cai's Algorithm (\% early stop: 0): \%pts/\%sel}\\
Dose Level(A$\backslash$B)	&	0.05	&	0.35	&	0.65	&	1	&	&	\\
0.1	&	0.031/0	&	0.008/0	&	0.009/0.004	&	0.001/0	&	&	\\
0.3	&	0.009/0	&	0.219/0.185	&	0.225/0.271	&	0.004/0.001	&	&	\\
0.6	&	0.013/0.002	&	0.299/0.399	&	0.116/0.136	&	0.016/0.002	&	&	\\
0.9	&	0.001/0	&	0.002/0	&	0.016/0	&	0.031/0	&	&	\\
\hline
\\ \\


==> sc2_own.tex <==
\hline
\multicolumn{7}{c}{\textbf{Scenario 2} \% early stop: 0} \\
\multicolumn{7}{l}{\textit{1.} Quadratic; Efficacy peaks in the left side of MTD; Insertion is not needed}\\
\hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(-1.38,1.38,1.01)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	-1.392(0.285)	&	1.13(0.913)	&	1.031(0.839)	\\	
\hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(1.44,-1.03,-0.5,-9.52,-6.64)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	-0.952(0.53)	&	0.994(1.335)	&	-0.432(0.896)	&	.	&	.	\\	
Quadratic of agent A	&	&	1.794(0.57)	&	-0.88(2.51)	&	1.359(1.516)	&	-34.834(13.359)	&	.	\\	
Quadratic of agent B	&	&	2.413(0.674)	&	1.46(1.583)	&	-0.688(2.026)	&	.	&	-40.72(14.957)	\\	
Quadratic of both agents	&	&	1.776(0.509)	&	-0.332(1.928)	&	-0.275(1.686)	&	-15.634(8.089)	&	-11.464(5.703)	\\	
\hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 0.1 \%$	&	\multicolumn{2}{c}{$ 7.4 \%$}	&	\multicolumn{2}{c}{$ 3.2 \%$}	&	\multicolumn{2}{c}{$ 89.3 \%$}	\\	
\hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.1	&	0.45	&	0.75	&	1	&	&	\\	
0.1	&	0.05/0.02&	0.08/0.14&	0.12/0.1&	0.15/0.02&&\\
0.45	&	0.1/0.32&	0.15/0.79&	0.21/0.72&	0.27/0.3&&\\
0.7	&	0.16/0.18&	0.23/0.64&	0.3/0.55&	0.38/0.17&&\\
0.9	&	0.22/0.02&	0.31/0.14&	0.39/0.1&	0.47/0.02&&\\
\hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(0.442,0.477),   BMS:\%ins=15.6\% }\\
\multicolumn{7}{c}{Dose inserted: 0.533(0.146), 0.575(0.142);  Dose selected: 0.454(0.051), 0.466(0.093)}\\
\hline
Dose Level(A$\backslash$B)	&	0.1	&	0.45	&	0.75	&	1	&	Dose inserted	&	Dose selected	\\
0.1	&	0.031/0.001	&	0.022/0.006	&	0.003/0.002	&	0.001/0	&	0.042/0.063	&	0.611/	\\
0.45	&	0.046/0.021	&	0.633/0.835	&	0.051/0.054	&	0.004/0	&	&	\\
0.7	&	0.003/0	&	0.032/0.018	&	0.032/0	&	0.019/0	&	&	\\
0.9	&	0/0	&	0.003/0	&	0.021/0	&	0.057/0	&	&	\\
\hline
\multicolumn{7}{l}{\textit{7.} Dose Allocation and Selection Percentages for Cai's Algorithm (\% early stop: 0): \%pts/\%sel}\\
Dose Level(A$\backslash$B)	&	0.1	&	0.45	&	0.75	&	1	&	&	\\
0.1	&	0.032/0.001	&	0.017/0.002	&	0.005/0.001	&	0.002/0	&	&	\\
0.45	&	0.042/0.023	&	0.706/0.91	&	0.053/0.05	&	0.003/0	&	&	\\
0.7	&	0.007/0	&	0.034/0.012	&	0.032/0.001	&	0.015/0	&	&	\\
0.9	&	0.002/0	&	0.003/0	&	0.017/0	&	0.03/0	&	&	\\
\hline
\\ \\


==> sc3_own.tex <==
\hline
\multicolumn{7}{c}{\textbf{Scenario 3} \% early stop: 0.001} \\
\multicolumn{7}{l}{\textit{1.} Quadratic; Efficacy peaks in the right side of MTD; Only a few dose combos are tolerable; Insertion is needed.}\\
\hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(-0.25,2.22,2.05)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	-0.208(0.346)	&	1.994(0.956)	&	1.792(0.794)	\\	
\hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(1.69,2.87,0.14,-8.24,-3.75)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	1.025(0.797)	&	6.108(2.633)	&	0.137(0.842)	&	.	&	.	\\	
Quadratic of agent A	&	&	1.126(0.538)	&	2.209(1.189)	&	1.122(0.856)	&	-9.821(4.077)	&	.	\\	
Quadratic of agent B	&	&	1.394(0.635)	&	4.565(1.637)	&	-0.177(1.244)	&	.	&	-8.127(3.87)	\\	
Quadratic of both agents	&	&	1.891(0.62)	&	2.821(1.347)	&	0.212(0.966)	&	-9.364(3.768)	&	-5.297(2.104)	\\	
\hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 0.7 \%$	&	\multicolumn{2}{c}{$ 24 \%$}	&	\multicolumn{2}{c}{$ 2.2 \%$}	&	\multicolumn{2}{c}{$ 73 \%$}	\\	
\hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.2	&	0.5	&	0.75	&	1	&	&	\\	
0.05	&	0.07/0.03&	0.15/0.1&	0.27/0.1&	0.44/0.04&&\\
0.25	&	0.11/0.27&	0.24/0.58&	0.4/0.58&	0.59/0.34&&\\
0.55	&	0.24/0.62&	0.44/0.86&	0.62/0.86&	0.78/0.69&&\\
0.9	&	0.48/0.24&	0.69/0.54&	0.82/0.54&	0.91/0.3&&\\
\hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(0.41,0.332),   BMS:\%ins=29.6\% }\\
\multicolumn{7}{c}{Dose inserted: 0.323(0.184), 0.286(0.148);  Dose selected: 0.38(0.145), 0.336(0.151)}\\
\hline
Dose Level(A$\backslash$B)	&	0.2	&	0.5	&	0.75	&	1	&	Dose inserted	&	Dose selected	\\
0.05	&	0.032/0.005	&	0.034/0.01	&	0.025/0.002	&	0.011/0	&	0.075/0.189	&	0.408/	\\
0.25	&	0.115/0.085	&	0.27/0.356	&	0.034/0.011	&	0.018/0.001	&	&	\\
0.55	&	0.222/0.323	&	0.029/0.016	&	0.031/0	&	0.023/0	&	&	\\
0.9	&	0.013/0.002	&	0.016/0	&	0.023/0	&	0.029/0	&	&	\\
\hline
\multicolumn{7}{l}{\textit{7.} Dose Allocation and Selection Percentages for Cai's Algorithm (\% early stop: 0): \%pts/\%sel}\\
Dose Level(A$\backslash$B)	&	0.2	&	0.5	&	0.75	&	1	&	&	\\
0.05	&	0.032/0.008	&	0.034/0.005	&	0.023/0.008	&	0.012/0	&	&	\\
0.25	&	0.117/0.079	&	0.285/0.367	&	0.037/0.023	&	0.009/0	&	&	\\
0.55	&	0.32/0.499	&	0.033/0.01	&	0.031/0	&	0.018/0	&	&	\\
0.9	&	0.013/0.001	&	0.007/0	&	0.009/0	&	0.023/0	&	&	\\
\hline
\\ \\


==> sc4_own.tex <==
\hline
\multicolumn{7}{c}{\textbf{Scenario 4} \% early stop: 0.086} \\
\multicolumn{7}{l}{\textit{1.} Quadratic; Efficacy peaks in the right side of MTD; All dose are overly toxic; Insertion is needed.}\\
\hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(0.51,1.03,0.67)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	0.639(0.475)	&	1.039(0.592)	&	0.701(0.488)	\\	
\hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(0.69,-3.2,-1.76,-4.8,-2.93)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	1.209(0.825)	&	1.251(1.059)	&	0.453(0.911)	&	.	&	.	\\	
Quadratic of agent A	&	&	0.487(0.622)	&	-3.273(1.669)	&	0.286(0.786)	&	-5.286(1.899)	&	.	\\	
Quadratic of agent B	&	&	0.857(0.699)	&	0.997(0.911)	&	-2.232(1.488)	&	.	&	-3.727(1.782)	\\	
Quadratic of both agents	&	&	0.724(0.654)	&	-2.92(1.58)	&	-1.58(1.289)	&	-4.749(1.756)	&	-2.704(1.436)	\\	
\hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 1.5 \%$	&	\multicolumn{2}{c}{$ 18.3 \%$}	&	\multicolumn{2}{c}{$ 6.8 \%$}	&	\multicolumn{2}{c}{$ 68.7 \%$}	\\	
\hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.4	&	0.6	&	0.8	&	1	&	&	\\	
0.4	&	0.38/0.72&	0.45/0.76&	0.51/0.62&	0.57/0.25&&\\
0.6	&	0.48/0.76&	0.55/0.8&	0.61/0.66&	0.67/0.29&&\\
0.8	&	0.58/0.48&	0.64/0.53&	0.7/0.36&	0.75/0.11&&\\
1	&	0.67/0.06&	0.73/0.07&	0.78/0.04&	0.82/0.01&&\\
\hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(0.304,0.262),   BMS:\%ins=92.5\% }\\
\multicolumn{7}{c}{Dose inserted: 0.354(0.219), 0.354(0.231);  Dose selected: 0.242(0.073), 0.245(0.09)}\\
\hline
Dose Level(A$\backslash$B)	&	0.4	&	0.6	&	0.8	&	1	&	Dose inserted	&	Dose selected	\\
0.4	&	0.081/0.033	&	0.025/0	&	0.018/0	&	0.008/0	&	0.678/0.967	&	0.208/	\\
0.6	&	0.023/0	&	0.032/0	&	0.015/0	&	0.005/0	&	&	\\
0.8	&	0.014/0	&	0.015/0	&	0.026/0	&	0.013/0	&	&	\\
1	&	0.006/0	&	0.004/0	&	0.013/0	&	0.024/0	&	&	\\
\hline
\multicolumn{7}{l}{\textit{7.} Dose Allocation and Selection Percentages for Cai's Algorithm (\% early stop: 0.603): \%pts/\%sel}\\
Dose Level(A$\backslash$B)	&	0.4	&	0.6	&	0.8	&	1	&	&	\\
0.4	&	0.568/1	&	0.066/0	&	0.033/0	&	0.018/0	&	&	\\
0.6	&	0.064/0	&	0.04/0	&	0.03/0	&	0.009/0	&	&	\\
0.8	&	0.034/0	&	0.028/0	&	0.034/0	&	0.016/0	&	&	\\
1	&	0.018/0	&	0.007/0	&	0.011/0	&	0.023/0	&	&	\\
\hline
\\ \\


==> sc5_own.tex <==
\hline
\multicolumn{7}{c}{\textbf{Scenario 5} \% early stop: 0} \\
\multicolumn{7}{l}{\textit{1.} Quadratic; All dose are safe; The dose range only covers the bottom-left corner of the efficacy-dose curve. Insertion is needed.}\\
\hline
\multicolumn{7}{l}{\textit{2.} Toxicity Parameter Estimation, True $(\alpha_0,\alpha_1,\alpha_2)=(-2.8,0.77,0.52)$}  \\
&	&	&	&	$\hat{\alpha_0}$	&	$\hat{\alpha_1}$	&	$\hat{\alpha_2}$	\\	
&	&	&	&	-3.115(0.808)	&	0.924(0.976)	&	0.869(0.932)	\\	
\hline
\multicolumn{7}{l}{\textit{3.} Efficacy Parameter Estimation,True $(\beta_0,\beta_1,\beta_2,\beta_3,\beta_4)=(-2.86,3.56,2.22,-1.2,-0.73)$} \\
&	&	$\hat{\beta_0}$	&	$\hat{\beta_1}$	&	$\hat{\beta_2}$	&	$\hat{\beta_3}$	&	$\hat{\beta_4}$	\\	
Linear	&	&	-3.671(1.283)	&	3.062(1.935)	&	2.93(1.762)	&	.	&	.	\\	
Quadratic of agent A	&	&	-4.262(1.622)	&	3.814(2.555)	&	3.031(1.847)	&	0.318(2.519)	&	.	\\	
Quadratic of agent B	&	&	-4.078(1.506)	&	3.599(2.145)	&	3.006(2.131)	&	.	&	-0.05(2.547)	\\	
Quadratic of both agents	&	&	-4.597(1.578)	&	4.238(2.504)	&	3.108(2.04)	&	0.372(2.612)	&	-0.363(2.384)	\\	
\hline
\multicolumn{7}{l}{\textit{4.} Model Selection percentages}	\\	
Linear	&	\multicolumn{2}{c}{Quadratic of agent A}	&	\multicolumn{2}{c}{Quadratic of agent B}	&	\multicolumn{2}{c}{Quadratic of both agents}	\\	
$ 25.4 \%$	&	\multicolumn{2}{c}{$ 23.9 \%$}	&	\multicolumn{2}{c}{$ 23.2 \%$}	&	\multicolumn{2}{c}{$ 27.5 \%$}	\\	
\hline
\multicolumn{7}{l}{\textit{5.} True Toxicity and Efficacy Probability: Tox/Eff}	\\	
Dose Level (A$\backslash$B)	&	0.05	&	0.15	&	0.25	&	0.35	&	&	\\	
0.05	&	0.03/0&	0.03/0&	0.04/0.01&	0.05/0.01&&\\
0.15	&	0.04/0.01&	0.05/0.02&	0.05/0.04&	0.07/0.07&&\\
0.25	&	0.05/0.02&	0.06/0.06&	0.07/0.14&	0.09/0.24&&\\
0.35	&	0.07/0.06&	0.08/0.16&	0.1/0.31&	0.11/0.46&&\\
\hline
\multicolumn{7}{l}{\textit{6.} Dose Allocation and Selection Percentages \%pts/\%sel}	\\	
\multicolumn{7}{c}{BODC=(0.474,0.472),   BMS:\%ins=11.1\% }\\
\multicolumn{7}{c}{Dose inserted: 0.443(0.205), 0.243(0.166);  Dose selected: 0.358(0.053), 0.345(0.041)}\\
\hline
Dose Level(A$\backslash$B)	&	0.05	&	0.15	&	0.25	&	0.35	&	Dose inserted	&	Dose selected	\\
0.05	&	0.031/0	&	0.007/0	&	0.008/0	&	0.016/0.001	&	0.025/0.051	&	0.625/	\\
0.15	&	0.007/0	&	0.031/0	&	0.016/0	&	0.021/0.002	&	&	\\
0.25	&	0.008/0	&	0.016/0	&	0.033/0.001	&	0.045/0.009	&	&	\\
0.35	&	0.022/0	&	0.028/0.002	&	0.068/0.029	&	0.618/0.905	&	&	\\
\hline
\multicolumn{7}{l}{\textit{7.} Dose Allocation and Selection Percentages for Cai's Algorithm (\% early stop: 0): \%pts/\%sel}\\
Dose Level(A$\backslash$B)	&	0.05	&	0.15	&	0.25	&	0.35	&	&	\\
0.05	&	0.032/0.001	&	0.014/0	&	0.016/0.001	&	0.024/0.001	&	&	\\
0.15	&	0.013/0	&	0.032/0	&	0.024/0	&	0.028/0.003	&	&	\\
0.25	&	0.017/0.001	&	0.025/0	&	0.04/0.006	&	0.071/0.051	&	&	\\
0.35	&	0.035/0.006	&	0.045/0.023	&	0.139/0.162	&	0.447/0.745	&	&	\\
\hline
\\ \\


==> time.tex <==
\hline
Scenario&Algorithm&Mean(Sd)&Min$\sim$Max&p-value%\footnote{$^{**}$ stands for p-value less than 0.0001, and $^*$ stands for p-value less than 0.05.}
\\
\hline
Scenario 1&cohort divison&927.53(185.32)&346 $\sim$ 1076&$<0.0001^{**}$\\
&single cohort&1037.89(59.9)&558 $\sim$ 1077&\\
Scenario 2&cohort divison&914.34(203.19)&367 $\sim$ 1075&$<0.0001^{**}$\\
&single cohort&1030.54(76.2)&495 $\sim$ 1074&\\
Scenario 3&cohort divison&622.82(172.78)&26 $\sim$ 1062&$<0.0001^{**}$\\
&single cohort&1017.16(84.52)&26 $\sim$ 1071&\\
Scenario 4&cohort divison&898.55(234.54)&6 $\sim$ 1067&$<0.0001^{**}$\\
&single cohort&944.86(249.64)&6 $\sim$ 1073&\\
Scenario 5&cohort divison&1045.27(61.43)&522 $\sim$ 1081&0.2376\\
&single cohort&1050.79(46.31)&599 $\sim$ 1077&\\
Scenario 6&cohort divison&910.56(205.81)&28 $\sim$ 1073&$<0.0001^{**}$\\
&single cohort&1025.39(80.2)&28 $\sim$ 1072&\\
Scenario 7&cohort divison&986.98(151.56)&357 $\sim$ 1076&$<0.0001^{**}$\\
&single cohort&1036.87(68.52)&522 $\sim$ 1077&\\
Scenario 8&cohort divison&1011.31(127.67)&362 $\sim$ 1078&0.03$^{*}$\\
&single cohort&1034.41(77.74)&523 $\sim$ 1079&\\
Scenario 9&cohort divison&962.51(144.38)&350 $\sim$ 1079&$<0.0001^{**}$\\
&single cohort&1043.68(48.29)&534 $\sim$ 1076&\\
Scenario 10&cohort divison&977.7(145.86)&23 $\sim$ 1075&$<0.0001^{**}$\\
&single cohort&1037.96(68.01)&23 $\sim$ 1077&\\
\hline

